Provable Tensor Methods for Learning Mixtures of Generalized Linear Models

We consider the problem of learning mixtures of generalized linear models (GLM) which arise in classification and regression problems. Typical learning approaches such as expectation maximization (EM) or variational Bayes can get stuck in spurious local optima. In contrast, we present a tensor decomposition method which is guaranteed to correctly recover the parameters. The key insight is to employ certain feature transformations of the input, which depend on the input generative model. Specifically, we employ score function tensors of the input and compute their cross-correlation with the response variable. We establish that the decomposition of this tensor consistently recovers the parameters, under mild non-degeneracy conditions. We demonstrate that the computational and sample complexity of our method is a low order polynomial of the input and the latent dimensions.

==> overview_Mixture.tex <==
\subsection{Toy Example: Gaussian Mixture Input and single GLM} \label{sec:overview}

We now exhibit our results for the case where the input $x$ is a mixture of spherical Gaussians.  Let $x = Ah + z$, where $h\in \{e_1, \ldots, e_k\}$ is the choice variable, and for simplicity, let $z \sim \Nc(0, I)$ for all components. In this case,  the score function is given by \beq -\nabla_x \log f(x) = x- A \Ebb[h|x], \quad x = Ah +z, \, z \sim \Nc(0, I).\label{eqn:fisherscore-mixture}\eeq
Note that $E[h|x]$ is the posterior estimation of the mean, given $x$. In other words, the score function centers the input with the mean vectors which are weighted by the posterior. Intuitively, since we do not observe $h$, this is the right way to center our data.



Now let us look at the associative model of label $y$ given input  $x$. First consider the case, where $y$ is generated from a single GLM model, $ \Ebb[y|x] = g( \inner{ u,x})$, for some non-linear activation function $g(\cdot)$ and $u$ is the weight vector for the classifier.  The classical Stein's lemma states the score function of the input acts as a differential operator
\beq -\Ebb[ y \cdot \nabla_x \log f(x)] =  \Ebb[ \nabla_x g( \inner{ u,x})]. \eeq
Applying it to Gaussian mixture input in \eqref{eqn:fisherscore-mixture}, for a single GLM model, we have
\beq\label{eqn:singleGLM} -\Ebb[ y \cdot \nabla_x \log f(x)]= \Ebb\left[ y \cdot \left(x- A \Ebb[h|x]\right) \right] = \Ebb[ \nabla_x g( \inner{ u,x})]= \Ebb[g'] \cdot u.\eeq Thus, we obtain the weight vector $u$ of the GLM model by using the first order cross-moment between the label $y$ and the score function.

Several challenges arise when we want to extend the above framework to the mixture of GLMs. In this case, we have
\beq \Ebb[ y| x, \tilde{h}] = g\left(\inner{U\tilde{h}, x} \right),\eeq where $\tilde{h}\in \{e_1, \ldots, e_{\tilde{k}}\}$ is the choice variable for the classifier and $U$ is the matrix that consists of the weight vectors. The first order moment now is given by the weighted combination of the weight vectors. Thus, we need higher order moments for learning. To this end, we utilize higher order differential operators, which can be constructed recursively using higher order score function\aacomment{cite us}. Using this, we obtain the third order expected derivative of the label as a function of the input. We establish that this tensor has a CP decomposition, where each component corresponds to the weight vector of a component GLM.  Details can be found in Section~\ref{section:results}.

   

==> summary_mixture.tex <==
\subsection{Summary of Results}

We employ the generalized linear model (GLM) framework for modeling labels $y$ as a function of either of observed features $x$ or hidden ones $h$. In the simplest setting, we have $\Ebb[y|x] = g(\inner{u_h,x})$. Intuitively, this is similar to the crowd sourcing problem. Where people classify the features based on their personal opinion and we want to learn people's perception given the features and the labels. In absence of hidden variables, Fisher kernels can be utilized to learn the parameters. However, here we are considering the hidden variables for a more precise modeling. 

For learning mixture of classifiers, first order moment does not help in learning the classifiers. however, we can learn the classifiers using the third order moment.  This is moment-based analysis as opposed to maximum likelihood analysis and that is the reason this approach is computationally tractable.

We employ the tensor decomposition on moment tensors involving labels and functions of the observed features. In contrast, to optimization frameworks which employ a loss function, our method aims to learn the parameters through these moment tensors. We can always employ the results from the tensor method as initializers for optimizing any desired loss function. This has been done in the generative case. Also, we can employ the learned vectors through tensor methods for constructing discriminative features and training other classifiers.

